Writing on Dirty Paper with Resizing and its Application to Quasi-Static Fading Broadcast Channels

This paper studies a variant of the classical problem of ``writing on dirty paper'' in which the sum of the input and the interference, or dirt, is multiplied by a random variable that models resizing, known to the decoder but not to the encoder. The achievable rate of Costa's dirty paper coding (DPC) scheme is calculated and compared to the case of the decoder's also knowing the dirt. In the ergodic case, the corresponding rate loss vanishes asymptotically in the limits of both high and low signal-to-noise ratio (SNR), and is small at all finite SNR for typical distributions like Rayleigh, Rician, and Nakagami. In the quasi-static case, the DPC scheme is lossless at all SNR in terms of outage probability. Quasi-static fading broadcast channels (BC) without transmit channel state information (CSI) are investigated as an application of the robustness properties. It is shown that the DPC scheme leads to an outage achievable rate region that strictly dominates that of time division.

==> Makefile <==
 # LaTeX -*-Makefile-*-
#
# Here's what this Makefile gives you:
#
# make dvi	- Generates the DVI file, suitable for previewing
# make ps	- Generates a postscript file suitable for printing
# make pdf	- Generates a PDF file suitable for viewing/printing
# make all	- Generates DVI, postscript, and PDF files
# make clean	- Removes some intermediate files
# make squeaky	- Removes all generated PS, DVI, and PDF files
#

#
# INSTRUCTIONS:
# -------------
#
# This first section contains macros whose values that you need to
# fill in.
#

# MAIN_TEX: In order to build your thesis/dissertation, fill in the
# MAIN_TEX macro with the name of your main .tex file -- the one that
# you invoke LaTeX on.

MAIN_TEX	= wenyi_isit07.tex

# CHAP_CITE_TEX: Some departments require bibliographies for each
# chapter.  If your department only requires a single bibliography at
# the end of the work, leave this macro blank and go on to
# OTHER_SRC_FILES, below.

# If your department does require chapter bibliographies, put the
# filenames of your chapters in this macro (and do *not* list them
# again in OTHER_SRC_FILES, below).  You will also need to use the
# "chapterbib" classfile -- see the sample_ndthesis.tex for an
# example.  You will also need to remove the \bibliographystyle{} and
# \bibliography{} commands from the top-level file
# (sample_ndthesis.tex), and append them to the end of the files
# listed in CHAP_CITE_TEX.

CHAP_CITE_TEX	= 

# OTHER_SRC_FILES: Put in the names of all the other files that your
# thesis depends on (e.g., other .tex files, .eps figures, etc.) in
# the OTHER_SRC_FILES macro.  This is ensure that whenever one of the
# "other" files changes, "make" will rebuild your paper properly.  You
# should *not* list any files in this macro that were already listed
# in CHAP_CITE_TEX, above.

OTHER_SRC_FILES	= shiva.bib rv_defs1.tex 

# You should not need to change these, but just in case...

#LATEX		= /usr/local/src/tex/bin/latex
#DVIPS		= /usr/local/src/tex/bin/dvips 
LATEX		= latex
DVIPS		= dvips


#########################################################################
#
# You should not need to edit below this line
#
#########################################################################

.SUFFIXES: .tex .dvi .ps .pdf

CHAP_CITE	= $(CHAP_CITE_TEX:.tex=)
MAIN_DVI	= $(MAIN_TEX:.tex=.dvi)
MAIN_PS		= $(MAIN_TEX:.tex=.ps)
MAIN_PDF	= $(MAIN_TEX:.tex=.pdf)

#
# Some common target names
# Note that the default target is "ps"
#

ps: $(MAIN_PS) 
postscript: ps
pdf: $(MAIN_PDF)
acrobat: pdf
dvi: $(MAIN_DVI)

thesis: ps
all: pdf

#
# Make the dependencies so that things build when they need to
#

$(MAIN_PS): $(MAIN_DVI)
$(MAIN_DVI): $(MAIN_TEX) $(CITE_TEX) $(OTHER_SRC_FILES)
$(MAIN_PDF): $(MAIN_DVI)

#
# General rules
#

.tex.dvi:
	@$(LATEX) $*
	@if ( grep 'LaTeX Warning: Label(s) may' $*.log > /dev/null ); \
	then $(LATEX) $* ; else :; fi
	@ if ( grep 'Writing index file' $*.log > /dev/null ); \
	then makeindex $* ; $(LATEX) $* ; fi
	@-if ( grep 'LaTeX Warning: Citation' $*.log > /dev/null ); then \
	  if test "$(CHAP_CITE)" ; then \
	    for file in bogus $(CHAP_CITE) ; do \
	      if test "$$file" != "bogus"; then \
		echo "RUNNING BIBTEX ON FILE: $$file"; \
		bibtex $$file ; \
	      fi ; \
	    done ; \
	  else \
	    echo "RUNNING BIBTEX ON FILE: $*"; \
	    bibtex $* ; \
	  fi ; \
	  $(LATEX) $* ; \
	fi
	@if ( grep 'LaTeX Warning: Label(s) may' $*.log > /dev/null || \
	      grep 'Rerun LaTeX' $*.log > /dev/null || \
	      grep 'LaTeX Warning: Citation' $*.log > /dev/null); \
	then $(LATEX) $* ; else :; fi
	@if ( grep 'LaTeX Warning: Label(s) may' $*.log > /dev/null || \
	      grep 'Rerun LaTeX' $*.log > /dev/null || \
	      grep 'LaTeX Warning: Citation' $*.log > /dev/null); \
	then $(LATEX) $* ; else :; fi
	@if ( grep 'LaTeX Warning: Label(s) may' $*.log > /dev/null || \
	      grep 'Rerun LaTeX' $*.log > /dev/null || \
	      grep 'LaTeX Warning: Citation' $*.log > /dev/null); \
	then $(LATEX) $* ; else :; fi

.dvi.ps:
	$(DVIPS) -Pps-type1 -o $*.ps $*

.dvi.pdf:
	dvipdf $*.dvi $*.pdf
#	distill -maxsubsetpct 99 -subsetfonts on -pairs $*.ps $*.pdf

#
# Standard targets
#

clean:
	/bin/rm -f *~ *.bak *%

squeaky:
	/bin/rm -f *.log *.aux *.dvi *.blg *.toc  *.lof *.lot \ $(MAIN_PDF)$ $(MAIN_PS) $(MAIN_DVI)


==> ltx <==
#!/usr/bin/perl
$a0=shift;

	$comm1=join('',"latex -interaction errorstopmode ",$a0,".tex");
	print "$comm1\n\n";
	system($comm1);
	print "$comm1\n\n";
	$comm4=join('',"latex -interaction errorstopmode ",$a0,".tex");
	print "$comm4\n\n";
	system($comm4);
	print "$comm4\n\n";
	$comm2=join('',"dvips ","-Ppdf -tletter -G0 -q ",$a0,".dvi -o ",$a0,".ps");
	print "$comm2\n\n";
	system($comm2);
	
	$comm3=join('',"gs -q -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=letter -sOutputFile=",$a0,".pdf ",$a0,".ps");
	print "$comm3\n\n";
	system($comm3);
	

	
#	$comm3=join('',"ps2pdf ",$a0,".ps ",$a0,".pdf");
#	system($comm3);
#	print "$comm3\n\n";


